Cone-Copositive Lyapunov Functions for Complementarity Systems: Converse Result and Polynomial Approximation

This article establishes the existence of Lyapunov functions for analyzing the stability of a class of state-constrained systems, and it describes algorithms for their numerical computation. The system model consists of a differential equation coupled with a set-valued relation which introduces discontinuities in the vector field at the boundaries of the constraint set. In particular, the set-valued relation is described by the subdifferential of the indicator function of a closed convex cone, which results in a cone-complementarity system. The question of analyzing stability of such systems is addressed by constructing cone-copositive Lyapunov functions. As a first analytical result, we show that exponentially stable complementarity systems always admit a continuously differentiable cone-copositive Lyapunov function. Putting some more structure on the system vector field, such as homogeneity, we can show that the aforementioned functions can be approximated by a rational function of cone-copositive homogeneous polynomials. This later class of functions is seen to be particularly amenable for numerical computation as we provide two types of algorithms for precisely that purpose. These algorithms consist of a hierarchy of either linear or semidefinite optimization problems for computing the desired cone-copositive Lyapunov function. Some examples are given to illustrate our approach.

==> converseConv.tex <==
% !TEX root = sosCertEVIs.tex
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Stability Conditions}\label{sec:stabcon}

\subsection{Stability Conditions}
We may now define as in \cite{GoelBrog04},\cite{GoelMotr03} the stability of the trivial solution. The stationary solution $0$ is stable if small perturbations of the initial condition $x(t_{0})=0$ lead to solutions remaining in the neighborhood of $0$ for all $t \ge t_{0}$, precisely:
\begin{defn}
The equilibrium point $x=0$ is said to be stable in the sense of Lyapunov if for every $\epsilon > 0$ there exists $\beta=\beta(\epsilon)>0$ such that for any $x_{0} \in \dom(\partial\varphi)$ with $\|x_{0}\| \le \beta$ the solution $x(.;t_{0},x_{0})$ of problem $P(t_{0},x_{0})$ satisfies
\[
\|x(t,t_{0},x_{0})\| \le \epsilon, \forall t \ge t_{0}
\]
\end{defn}
\begin{defn}
The equilibrium point $x=0$ is asymptotically stable if it is stable and there exists $\delta >0$ such that for any $x_{0} \in \dom(\partial\varphi)$ with $\|x_{0}\| \le \delta$ the solution $x(.;t_{0},x_{0})$ of problem $P(t_{0},x_{0})$ satisfies
\[
\lim\limits_{t \rightarrow +\infty} \|x(t,t_{0},x_{0})\| =0
\]
\end{defn}
\begin{defn}
The equilibrium point $x=0$ is unstable if it is not stable, i.e., there exists $\epsilon >0$ such that for any $\beta>0$, one may find $x_{0} \in \dom(\partial\varphi)$ with $\|x_{0}\| \le \beta$ and $\bar{t} \ge t_{0}$ such that the solution $x(.;t_{0},x_{0})$ of problem $P(t_{0},x_{0})$ satisfies
\[
 \|x(t,t_{0},x_{0})\| > \epsilon
\]
\end{defn}
Let us now give a general theorem of stability conditions as in \cite{GoelMotr03} in terms of Lyapunov function $V \in C^1(\R^n,\R)$.
\begin{thm} (Stability conditions)\label{thm:stabConditions}
Suppose that the assumptions of Theorem~\ref{thm:existencesol} with condition ~\eqref{evi} hold and there exist $\sigma>0$ and $V \in C^1(\R^n,\R)$ such that\\
$(1)$
\[
V(x) \ge a(\|x\|), \enspace x \in \dom(\partial\varphi), \enspace \|x\| \le \sigma,
\]
with $a: [0,\sigma] \mapsto \R$ satisfying $a(t)>0$, $\forall$ $t \in [0,\sigma]$;\\
$(2)$ $V(0)=0$;\\
$(3)$ $\left\langle \nabla V(x),F(x)-w \right\rangle \le 0$, $x \in \dom(\partial \varphi)$, $\|x\| \le \sigma$, $w \in \partial\varphi(x)$, $t \ge t_{0}$.\\
Then the trivial solution of problem $P(t_{0},0)$ is stable.
\end{thm}


In this section, we will establish an existence result for Lyapunov function, that is, if the system is exponentially stable then there exists a Lyapunov function for such system. We will in particular focus in this paper on linear complementarity systems of the form:
\begin{subequations}\label{eq:defLCS}
\begin{gather}
    \dot x = Ax + \lambda \\
    K \ni x \perp \lambda \in K^\star
\end{gather}
\end{subequations}
and we let $K$ be a polyhedral defined as $K=\left\{x\in \R^n; Fx \ge 0\right\}$  where $F \in \R^{m \times n}$ is a matrix and $K^\star$ is the dual of $K$.
Our approach is inspired by several results on converse Lyapunov theorems for switched systems, \cite{DayaMart99, MasoBosc06} and complementarity systems \cite{CamlPang06}. The difficulty in generalizing the more conventional converse results comes from the fact that our Lyapunov functions is not smooth enough. Such converse theorems were addressed for complementarity systems in \cite{CamlPang06}, but here we modify there construction to show that there exists a copositive polynomial Lyapunov function for complementarity systems.


\begin{exam}[Constraints make the solution space nonlinear]
Consider the dynamical system \eqref{eq:defLCS} with $A = \begin{bmatrix}0 & 1\\-1 & 0\end{bmatrix}$, and let $x_1(0) = (a, 0)^\top$ and $x_2(0) = (0,b)^\top$. Let $x_i:\R\to \R^2$ be the solution starting with initial condition $x_i(0)$, $i = 1,2$; and let $z$ denote the solution starting with initial condition $x_1(0) + x_2(0)$. It can be checked that $z(t)$ does not equal $x_1(t) + x_2(t)$, for any $t > 0$.
\end{exam}

\begin{exam}[Constraints make the system GAS, even if $A$ is not Hurwitz]
Consider again the system \eqref{eq:defLCS} with $A = \begin{bmatrix} -1 & -2\\ -1 &-1\end{bmatrix}$. Clearly, the matrix $A$ is not Hurwitz since one of its eigenvalues has positive real part. However, it can be verified that there exists a Lyapunov function $V: \R^n \to \R$ satisfying the sufficient conditions given in Proposition~\ref{prop:}. Indeed, we can take $V(x) = x^\top P x$, with $P$ a copositive matrix, that is, $z^\top P z > 0$ for $z > 0$.
\end{exam}

\begin{assump}[leftmargin=*]
\item\label{a:dissA} The matrix \(A\) is dissipative, that is,
\[
A + A^\top \le 0.
\]
\item\label{a:diffVecField} The matrix $D$ is a $P$-matrix and the resulting vector field is directionally differentiable.
\end{assump}

\begin{thm}\label{thm:converseMain}
Consider the dynamical system \eqref{eq:defLCS}. There exists a homogeneous polynomial copositive Lyapunov function of degree $2$ for the complementarity systems.
\end{thm}

The proof of this theorem is a lengthy and technical affair and is carried out in Section~\ref{sec:proofConverse}.

\section{Proof of Theorem~\ref{thm:converseMain}}
\label{sec:proofConverse}

We start with the function $V : \R^n \to \R$, defined as
\[
V(z) = \int_{0}^\infty x(\tau;z)^\top x(\tau; z) \, d\tau
\]

The function $V$ is clearly continuous because of the continuous dependence of the solutions on the initial conditions.
\begin{lem}
The locally Lipschitz function $V$ is strictly decreasing along the solutions of the system.
\end{lem}
\begin{proof}
From the definition of $V$, with $x(0) = z$, it is seen that
\[
V(z) \ge \int_{0}^t x(\tau;z)^\top x(\tau;z) d\, \tau + \int_{0}^\infty x(\tau;x(t;z))^\top x(\tau;x(t;z)) \, d\,\tau
\]
and hence
\[
V(x(t)) - V(x(0)) \le - \int_{0}^t x(\tau;z)^\top x(\tau;z) d\, \tau.
\]
{\color{red}For $t$ sufficiently small, we also have that
\[
x(t) = z + t f + o (t)
\]
and this gives
\[
D V(z;v) \le - z^\top z
\]
which shows the strong decrease in the value of $V$.
}
\end{proof}


\subsection{Convexity and Lipschitz Continuity of $V$}

\begin{lem}
For every initial condition $z \ge 0$ and the solution $x(\tau;z)$ obtained from \eqref{eq:defLCS}, it holds that the mapping
\begin{equation}
x_0 \mapsto \|x(t;x_0)\|^2
\end{equation}
is strictly convex for each $t \ge 0$.
\end{lem}
\begin{proof}
Fix $t \ge 0$, and take $x_{1,0}$ and $x_{2,0}$ to be the two initial conditions in $\R_+^n$ with their corresponding solutions denoted by $x_1(t)$ and $x_2(t)$. For a fixed $\mu \in [0,1]$, let $y_0 = \mu x_{1,0} + (1-\mu) x_{2,0} \in \R_+^n$, and let $y(t)$ be the solution to system \eqref{eq:defLCS} with $y(0) = y_0$. To prove the lemma, we need to show that, for every $0 < \mu < 1$, $ \|y(t) \|^2 \le \mu \|x_{1}(t) \|^2 + (1-\mu) \|x_2(t) \|^2$. Toward this end, it follows from the system dynamics that
\[
\left\langle \frac{d y}{dt} (t) - f(y(t)), z - y(t) \right \rangle \ge 0
\]
Let $r > 0$ and $\tau = \lambda^d t$.
\paragraph{For $y$} the calculation of $\lambda^{2r}\frac{d}{d\tau}\|y(\tau) \|^2$ gives
\begin{align*}
& \lambda^{2r}\frac{d}{d\tau}\|y(\tau) \|^2 \\
& = 2 \lambda^{2r} \left\langle \frac{d y}{d\tau} (\tau), y(\tau) \right\rangle \\
& = 2 \lambda^{2r} \left\langle \frac{d y}{d\tau} (\tau) - \lambda^d f(y(\tau)), y(\tau) \right\rangle \\
& + 2 \lambda^{2r} \left\langle \lambda^d f(y(\tau)) , y(\tau) \right\rangle \\
& = 2 \left\langle \lambda^r \left( \frac{d y}{d\tau} (\tau) - \lambda^d f(y(\tau)) \right), \lambda^r y(\tau) \right\rangle \\
& +2 \lambda^{2r} \lambda^d \left\langle f(y(\tau)) , y(\tau) \right\rangle
\end{align*}
By the homogeneity of $f$, we obtain
\begin{multline*}
\lambda^{2r}\frac{d}{d\tau}\|y(\tau) \|^2 = 2 \underbrace{\left\langle \frac{d}{d\tau} \lambda^r y(\tau) - f(\lambda^r y(\tau)), \lambda^r y(\tau) \right\rangle}_{\textbf{(A)}} \\
+ 2 \lambda^{2r} \lambda^d \left\langle f(y(\tau)) , y(\tau) \right\rangle
\end{multline*}
Since $\lambda^r y(\tau)$ is a solution of the system, we obtain that $\textbf{(A)} = 0$ , which implies

\begin{equation}\label{ineq1}
\frac{d}{d\tau}\|y(\tau) \|^2 = 2 \lambda^d  y(\tau)^\top f(y(\tau))
\end{equation}

\paragraph{For $x_1$} Reasoning in the same way as before, the calculation of $\lambda^{2r} \lambda^d \frac{d}{d\tau}\|y(\tau) \|^2$ gives
\begin{align*}
& \lambda^{2r} \lambda^d \frac{d}{d\tau}\|x_1(\tau) \|^2 \\
& = 2 \lambda^{2r} \lambda^d \left\langle \frac{d x_1}{d\tau} (\tau), x_1(\tau) \right\rangle \\
%& = 2 \lambda^{2r} \lambda^d \left\langle \frac{d x_1}{d\tau} (\tau) - \lambda^d f(x_1(\tau)), x_1(\tau) \right\rangle \\
%& + 2 \lambda^{2r} \lambda^d \left\langle \lambda^d f(x_1(\tau)) , x_1 (\tau) \right\rangle \\
%& = 2 \lambda^d \left\langle \lambda^r ( \frac{d x_1}{d\tau} (\tau) - \lambda^d f(x_1(\tau))), \lambda^r x_1(\tau) \right\rangle \\
%& + 2 \lambda^{2r} \lambda^{2d} \left\langle f(x_1(\tau)) , x_1(\tau) \right\rangle \\
& = 2 \lambda^d \underbrace{\left\langle \frac{d}{d\tau} \lambda^r x_1(\tau) - f(\lambda^r x_1(\tau)), \lambda^r x_1(\tau) \right\rangle}_{\textbf{(B)}} \\
& + 2 \lambda^{2r} \lambda^{2d} \left\langle f(x_1(\tau)) , x_1(\tau) \right\rangle
\end{align*}

Since $\lambda^r x_1(\tau)$ is a solution of the system, we obtain $\textbf{(B)} = 0$. This implies

\begin{equation}\label{ineq2}
\lambda^d \frac{d}{d\tau}\|x_1(\tau) \|^2 = 2 \lambda^{2d} x_1(\tau)^\top f(x_1(\tau))
\end{equation}

\paragraph{For $x_2$} the calculation of $\lambda^{2r}\frac{d}{d\tau}\|y(\tau) \|^2$ gives
\begin{align*}
& \lambda^{2r} (1-\lambda^d) \frac{d}{d\tau}\|x_2(\tau) \|^2 \\
& = 2 \lambda^{2r} (1-\lambda^d) \left\langle \frac{d x_2}{d\tau} (\tau), x_2(\tau) \right\rangle \\
%& = 2 \lambda^{2r} (1-\lambda^d) \left\langle \frac{d x_2}{d\tau} (\tau) - \lambda^d f(x_2(\tau)), x_2(\tau) \right\rangle \\
%& + 2 \lambda^{2r} (1-\lambda^d) \left\langle \lambda^d f(x_2(\tau)) , x_2 (\tau) \right\rangle \\
%& = 2 (1-\lambda^d) \left\langle \lambda^r ( \frac{d x_2}{d\tau} (\tau) - \lambda^d f(x_2(\tau))), \lambda^r x_2(\tau) \right\rangle \\
%& + 2 \lambda^{2r} \lambda^d (1-\lambda^d) \left\langle f(x_2(\tau)) , x_2(\tau) \right\rangle \\
& = 2 (1-\lambda^d) \underbrace{\left\langle \frac{d}{d\tau} \lambda^r x_2(\tau) - f(\lambda^r x_2(\tau)), \lambda^r x_2(\tau) \right\rangle}_{\textbf{(C)}} \\
& + 2 \lambda^{2r} \lambda^d (1-\lambda^d) \left\langle f(x_2(\tau)) , x_2(\tau) \right\rangle
\end{align*}

Since $\lambda^r x_2(\tau)$ is a solution of the system, we get $\textbf{(C)} = 0$ , which implies

\begin{equation}\label{ineq3}
(1-\lambda^d) \frac{d}{d\tau}\|x_2(\tau) \|^2 = 2 \lambda^d (1-\lambda^d) x_2(\tau)^\top f(x_2(\tau))
\end{equation}

Combining these three inequalities, we get
\begin{multline}
\frac{d}{d \tau} \left( \|y(\tau) \|^2 - \lambda^d \|x_1(\tau) \|^2 - (1-\lambda^d) \|x_2(\tau) \|^2 \right )   \\
= 2 \lambda^d ( y(\tau)^\top f(y(\tau)) - \lambda^d x_1(\tau)^\top f(x_1(\tau))  \\
- (1-\lambda^d)x_2(\tau)^\top f(x_2(\tau))).
\end{multline}
Let $\alpha > 0$ be such that
\[
-\alpha \vert z \vert ^2 \le z^\top f(z) \le \alpha \vert z \vert^2
\]
which results in
\begin{multline}
2 \lambda^d (y(\tau)^\top f(y(\tau)) - \lambda^d x_1(\tau)^\top f(x_1(\tau)) -(1-\lambda^d) \\
x_2(\tau)^\top f(x_2(\tau)) ) \\
\le 2 \alpha \lambda^d  \left( \|y(\tau) \|^2 - \lambda^d \|x_1(\tau) \|^2 -
 (1-\lambda^d) \|x_2(\tau) \|^2 \right ).
\end{multline}
Hence, applying Gronwall's lemma, we get
\begin{multline}
\left( \|y(\tau) \|^2 - \lambda^d \|x_1(\tau) \|^2 - (1-\lambda^d) \|x_2(\tau) \|^2 \right ) \le \\
\epower{2 \alpha \lambda^d (t-t_0)} \left( \|y_0 \|^2 - \lambda^d \|x_{1,0} \|^2 - (1-\lambda^d) \|x_{2,0} \|^2 \right )
\end{multline}

Taking $\mu =\lambda^d \in [0,1]$ and since $y_0 = \mu x_{1,0} + (1-\mu) x_{2,0}$ and the function $\R^n \ni x \mapsto \|x\|^2$ is a convex function, we have
\[
\|y_0 \|^2 \le  \mu \|x_{1,0} \|^2 + (1-\mu) \|x_{2,0} \|^2
\]
and hence
\[
\|y(\tau) \|^2  \le \mu \|x_1(\tau) \|^2 + (1-\mu) \|x_2(\tau) \|^2
\]
which proves convexity of the desired map.


%Also, since $\lambda^r x_1(\lambda^d t)$ is a solution with $\tau_1 = \lambda^d t$, we have
%\[
%\lambda^{r+d} \left\langle \frac{d x_1}{dt} (\tau_1) - f(x_1(\tau_1)), v_1 - \lambda^r x_1(\tau_1) \right \rangle \ge 0
%\]
%and $(1-\lambda)^r x_2((1-\lambda)^d t)$ being a solution with $\tau_2 = (1-\lambda)^d t$ yields
%\[
%(1-\lambda)^{r+d} \left\langle \frac{d x_2}{dt} (\tau_2) - f(x_2(\tau_2)), v_2 - (1-\lambda)^r x_2(\tau_2) \right \rangle \ge 0
%\]
%Take \( z=0 \), \( v_1 = (1+\lambda^r) x_1(\tau_1) \) and \(v_2 = (1+(1-\lambda)^r) x_2(\tau_2) \), then
%\begin{multline}
%\frac{d}{dt} \left( \|y(t) \|^2 - \lambda^{r+d} \|x_1(\tau_1) \|^2 - (1-\lambda)^{r+d} \|x_2(\tau_2) \|^2 \right )  \le \\
% y(t)^\top f(y(t)) - \lambda^{r+d} x_1(\tau_1)^\top f(x_1(\tau_1)) \\
% - (1-\lambda)^{r+d} x_2(\tau_2)^\top f(x_2(\tau_2))
%\end{multline}
%Let $\alpha > 0$ be such that
%\[
%-\alpha \vert z \vert ^2 \le z^\top f(z) \le \alpha \vert z \vert^2
%\]
%which results in
%\begin{multline}
%y(t)^\top f(y(t)) - \lambda^{r+d} x_1(\tau_1)^\top f(x_1(\tau_1)) \\
%- (1-\lambda)^{r+d} x_2(\tau_2)^\top f(x_2(\tau_2)) \le \\
%\alpha  \left( \|y(t) \|^2 - \lambda^{r+d} \|x_1(\tau_1) \|^2 - (1-\lambda)^{r+d} \|x_2(\tau_2) \|^2 \right ).
%\end{multline}
%Hence, applying Gronwall's lemma, we get
%\begin{multline}
%\left( \|y(t) \|^2 - \lambda^{r+d} \|x_1(\tau_1) \|^2 - (1-\lambda)^{r+d} \|x_2(\tau_2) \|^2 \right ) \le \\
%\epower{\alpha(t-t_0)} \left( \|y_0 \|^2 - \lambda^{r+d} \|x_{1,0} \|^2 - (1-\lambda)^{r+d} \|x_{2,0} \|^2 \right )
%\end{multline}
%But since, $y_0 = \lambda x_{1,0} + (1-\lambda) x_{2,0}$ and the function $\R^n \ni x \mapsto \|x\|^2$ is a convex function, we have
%\[
%\|y_0 \|^2 \le  \lambda \|x_{1,0} \|^2 + (1-\lambda) \|x_{2,0} \|^2
%\]
%and hence
%\[
%\|y(t) \|^2  \le \lambda \|x_1(t) \|^2 + (1-\lambda) \|x_2(t) \|^2
%\]
%which proves convexity of the desired map.
\end{proof}



\subsection{Regularization of $V$}
The next step is to regularize $V$ so that we obtain a continuously differentiable Lyapunov function.

\begin{lem}\label{lem:smoothReg}
There exists a continuous differentiable function $\wt V$ which is strictly decreasing along the solutions of the system.
\end{lem}

\[
\wt V(z) = \int_{SO(n)} V (Rz) \psi (R) dR
\]
where $\psi$ is the mollifier $\int \psi(R) dR = 1$.

\begin{proof}[Proof of Lemma~\ref{lem:smoothReg}]

Introduce the perturbations of the system; do the regularization; and show that the regularized function is also decreasing.


By definition, $\wt V$ is continuously differentiable. We next show that the directional derivative of $\wt V$ along the system vector fields is negative definite. To do so, we need a bound on $\wt V(Rz) - \wt V(R(z+tf))$ for $t\ge 0$ sufficiently small, where $f(z)  = Az + \lambda_z$. To do so, we introduce the vector,
\[
v_z = Az + \frac{1}{h}\big( \proj_K(z+hAz) - (z+hAz) \big)
\]
for some $h>0$, so that
\[
v_z \in Az - \cN_K (\proj_K(z+hAz)).
\]
We will get the desired bounds by rewriting the difference as
\begin{multline*}
\wt V(R(z+tf)) - \wt V(Rz) = \wt V(R(z+tf)) - \wt V(R(z+tv)) \\
+ \wt V(R(z+tv)) - \wt V(Rx(t;z)) + \wt V(R x(t;z)) - V(Rz)
\end{multline*}
and getting a bound on each of the three difference terms on the right-hand side.

\paragraph{1\textsuperscript{st} term} The first term
\[
\wt V(R(z+tf)) - \wt V(R(z+tv))
\]
can be analyzed by using the convexity of $K$ and projection being contractive. In this regard, we first note that
\[
f - v = \lambda_z - \frac{1}{h}\big( \proj_K(z+hAz) - (z+hAz) \big)
\]
so that
\[
\vert f - v \vert = \vert \lambda_z \vert + \frac{1}{h} d_\cS (z+hAz) = O(1)
\]
for each $h > 0$.
With $\wt V$ being locally Lipschitz, we have the desired decay of $O(t^2)$.

\paragraph{2\textsuperscript{nd} term} Next, the term
\[
\wt V(R(z+tv)) - \wt V(Rx(t;z))
\]
{\color{red}can be analyzed from the following lemma:
\begin{lem}\label{lem:discEst}
For $h> 0$ sufficiently small,  it holds that
\begin{equation}\label{eq:estDiscConverse}
\norm{z+hv  - x(h;z)} \le O(h)
\end{equation}
\end{lem}
}
Under the estimate \eqref{eq:estDiscConverse}, and using the Lipschitz continuity of $V$, we get
\[
\wt V(R(z+tv)) - \wt V(Rx(t;z)) = O(t^2).
\]

\paragraph{3\textsuperscript{rd} Term}Finally, for the last term, we have the estimate that
\[
\wt V(R x(t;z)) - V(Rz) \le -\int_0^t x(\tau; R z)^\top x(\tau; R z) d\, \tau.
\]
Combining these estimates, we get
\begin{align*}
\lim_{t \to 0^+} \frac{\wt V(R(z+tf)) - \wt V(Rz)}{t} & \le - z^\top z + o(t)
\end{align*}
and hence $\tilde V$ is differentiable and its derivative is negative definite.
This ends Lemma~\ref{lem:smoothReg}
\end{proof}


\begin{proof}[Proof of Lemma~\ref{lem:discEst}] Let $\overline z = \proj_K(z+hAz)$ and introduce the function $\wt z: [0,h] \to \R^n$ given by
\[
\wt z (t) = \frac{t}{h} \overline z + \left(1-\frac{t}{h} \right) z.
\]
It is readily checked that $\dot{\wt z} = \frac{d}{dt} \tilde z = v_z$.
%so t$\wt z(t) = z + t v_z$, so that $\wt z(h) = $ and $\dot {\wt z} = v_z$.
From the definition of $v_z$ and $\overline z$, it follows that
\[
\left\langle \dot{\wt z} - Az, \overline z - \wt y\right\rangle \le 0, \quad \forall \, \wt y \in K,
\]
or equivalently,
\[
\left\langle \dot{\wt z} - Az, \wt z(t) - \wt y \right \rangle \le \left\langle v_z - Az, \overline z - \wt z(t)\right\rangle, \quad \forall \, \wt y \in K.
\]
Also, using the equation for $\dot x$, and recalling that $\lambda \in -\cN_K (x)$, we have
\[
\left\langle Ax(t) - \dot x (t), y - x(t) \right\rangle \le 0, \quad \forall \, y \in K
\]
for almost all $t \ge 0$. In the last two inequalities, letting $\wt y = x(t) \in K$ and $y = \wt z(t) \in K$, and summing them, we get
\begin{multline*}
\left\langle \dot{\wt z} - \dot x(t), \wt z (t) - x(t) \right\rangle \le \left\langle A (z - x(t)), \wt z (t) - x(t) \right\rangle \\
+  \left\langle v_z - Az, \overline z - \wt z(t)\right\rangle.
\end{multline*}
To bound the first term on the right-hand side, we observe that
\begin{align*}
\vert z - x(t) \vert & \le \vert z - \wt z(t) \vert + \vert \wt z (t) - x(t) \vert \\
& \le t \vert v_z \vert + \vert \wt z (t) - x(t) \vert
\end{align*}
For the second term, it is seen that
\[
\vert v_z - Az \vert = \frac{1}{h} d_K (z+hAz) = O(1)
\]
and
\[
\vert \overline z - \wt z(t) \vert \le h \left(1-\frac{t}{h} \right) \vert v_z \vert \le h \vert v_z \vert
\]
Consequently, for some constants $C_1, C_2 > 0$
\begin{align*}
& \quad \frac{1}{2} \frac{d}{d t} \vert x(t;z) - \wt z (t) \vert ^2 \\
& = \left\langle \dot{\wt z} - \dot x(t), \wt z (t) - x(t) \right\rangle \\
& \le C_1 h \vert v_z\vert \vert \wt z (t) - x(t) \vert + C_2 \vert \wt z (t) - x(t) \vert ^2 + C_3 h \vert v_z\vert \\
& \le C_1 h + C_2 \vert \wt z (t) - x(t) \vert ^2 + O(h^2)
\end{align*}
where the last inequality is obtained by applying the Young's inequality to the product term $h \vert v_z \vert \vert \wt z(t) - x(t) \vert $
\[
\vert \wt z(t) - x(t) \vert^2 \le C_1 h \vert v_z \vert^2 t + C_2 \int_0^t \vert \wt z(s) - x(s) \vert^2 \, ds
\]
Application of Gronwall's lemma yields
\[
\vert \wt z(t) - x(t) \vert^2 \le C_1 h \vert v_z \vert^2 t \exp(C_2 t)
\]
whence the estimate \eqref{eq:estDiscConverse} follows by taking $t = O(h)$.
\end{proof}


\subsection{Polynomial Approximation of Convex Level Sets}
As the final step to get a polynomial Lyapunov function from $\wt V$, we prove the following lemma:

\begin{lem}
Consider a function $W:\R^n \to \R$ which is continuously differentiable, strictly convex and homogenous of degree $d$. Let $f:\R^n \to \R^n$  be locally bounded such that $\left\langle \nabla W (x), f(x) \right\rangle < 0$.
Then there exists a polynomial $\wt W: \R^n \to \R$, of sufficiently high degree, such that,
\[
\left\langle \nabla \wt W (x), f(x) \right\rangle < 0.
\]
\end{lem}
\begin{proof}
We consider the function $W(x)=\sqrt{\wt V(x)}$, which is continuously differentiable, strictly convex and homogeneous of degree d, seen by the properties of $\wt V(x)$. Using that the set $\left\{ x ; W(x) < 1 \right\}$ is strictly convex and by approximating the level sets of $W$, we construct a polynomial Lyapunov function $\wt W: \R^n \to \R$.

For this reason, we have need of the following lemma that shows the continuity of the function $ \left\langle \nabla W(y), f(x) \right\rangle $ with respect to $x$, $y$, $f$.

\begin{lem}\label{lem:contproperty}
Let us introduce
\[
M := \min_{ x \in W^{-1}(1) f \in \textrm{LB}(\R^n)} [-\nabla W(x).f(x)]
\]
where $\textrm{LB}(\R^n)$ denotes the set of locally bounded functions from $\R^n$ to $\R^n$. For every $\epsilon \in (0,M)$, there exists $\delta \in (0,1)$ such that for every $x, y \in W^{-1}(1)$ and every $f \in \textrm{LB}(\R^n)$ with $\nabla W(y) . x > d- \delta$, we obtain
\[
\nabla W(y).f(x) < -\epsilon.
\]
\end{lem}

\begin{proof}[Proof of Lemma~\ref{lem:contproperty}]
First, since $W$ is continuous over a compact set and $f$ is locally bounded then $M$ is well defined. And since $W$ is a Lyapunov function then $M > 0$.


Using the homogeneity of $W$, it gives $ \nabla W (y). y = d. W(y)$ and by the reason of $W(y)=1$, we obtain
\[
\nabla W (y). y = d
\]
which implies
\[
\nabla W (y). x = d-\nabla W (y). (y-x),
\]
and then the assumption $\nabla W(y) . x > d- \delta$ is equivalent to $\nabla W (y). (y-x) < \delta$.

Interpreting by contradiction, suppose that there exists a sequence $(x_i,y_i,f_j)$ such that $\nabla W(y_i).f_i(x_i) \ge -\epsilon$ and $\nabla W (y_i). (y_i-x_i) \rightarrow 0$ as $j \rightarrow \infty $.
By Bolzano-Weierstrass theorem in real analysis, we can find a subsequence of $(x_i,y_i,f_j)$ that converges to $(\bar{x},\bar{y},\bar{f})$. As a consequence, by continuity we get $\nabla W(\bar{y}). \bar{f}(\bar{x}) \ge -\epsilon$ and $\nabla W (\bar{y}). (\bar{y}-\bar{x}) = 0$.

The equation $\nabla W (\bar{y}). (\bar{y}-\bar{x}) = 0$ means that $\bar{y}-\bar{x}$ belongs to the tangent space at $\bar{y}$ of the strictly convex set $W^{-1}([0,1])$. Moreover we have that $\bar{x}$ is also on the boundary of this set then it should be $\bar{y}=\bar{x}$. From this, we get a contradiction seeing that  $\nabla W(\bar{y}). \bar{f}(\bar{x})= \nabla W(\bar{x}). \bar{f}(\bar{x}) \le -M$.

\end{proof}
We take $\delta \in (0,1)$ compatible to some $\epsilon$ in the lemma~\ref{lem:contproperty}, and for every $y \in W^{-1}(1)$, let $B_y = \left\{x \in \R^n \vert\ \nabla W (y) . x > 1-\frac{\delta}{2} \right\}$ the open sets. We have $y \in B_y$ so $\left\{ B_y \right\}_{y \in W^{-1}(1)}$ is an open covering of $W^{-1}(1)$. And then we can find $y_1,...,y_N$ points of $W^{-1}(1)$ such that the union of $B_{y_k}$, $k=1,...,N$, covers $W^{-1}(1)$.

Let us define
\[
\wt W(x) = \sum_{k=1}^{N} (\nabla W (y_k).x)^{2p}.
\]
For a large integer $p$, we affirm that $\wt W$ is a polynomial Lyapunov function.

For $f \in \textrm{LB}(\R^n)$ and $x \in \R^n$ such that $x \ne 0$, we have
\[
\wt W(x) . f(x) = 2p \sum_{k=1}^{N} (\nabla W (y_k).x)^{2p-1} \nabla W (y_k) . f(x).
\]
We need to prove that $\left\langle \nabla \wt W (x), f(x) \right\rangle < 0$. Since we have homogeneity, we can prove it just for $x \in W^{-1}(1)$. Let us introduce
\[
K := \max_{ x,y \in W^{-1}(1) f \in \textrm{LB}(\R^n)} [-\nabla W(y).f(x)].
\]
If for some $k \in \left\{1,...,N\right\}$, we have $\vert \nabla W(y_k) . x \vert \le d - \delta$, then
\[
\vert(\nabla W (y_k).x)^{2p-1} \nabla W (y_k) . f(x) \vert \le (d-\delta)^{2p-1} K.
\]
In other way, if $d- \frac{\delta}{2} \ge \vert \nabla W (y_k) . x \vert > d- \delta$, then, we can use lemma~\ref{lem:contproperty}. Therefore the term in the summation is negative.

Since there exist at least two distinct indices $k_1$ and $k_2$ such that $x \in B_{y_{k_1}}$ and $-x \in B_{y_{k_2}}$, we have
\[
(\nabla W (y_{k_i}).x)^{2p-1} \nabla W (y_{k_i}) . f(x) < -(d- \frac{\delta}{2})^{2p-1} \epsilon.
\]
Finally, we obtain that
\begin{align*}
\nabla & \wt W (x) . Dx  < 2p \left(-2(d-\delta/ 2)^{2p-1} \epsilon + (N-2)(d-\delta)^{2p-1} K \right) \\
& = -4p(d-\delta / 2)^{2p-1} \epsilon \left( 1- \frac{K(N-2)}{2 \epsilon} \left (\frac{d-\delta}{d-\delta /2} \right)^{2p-1} \right).
\end{align*}
For $p$ large enough, the right-hand side of the previous inequality is negative. Then the theorem~\ref{thm:converseMain} is proved.

\end{proof}


